Generative vs. Predictive Models in Massive MIMO Channel Prediction

Massive MIMO (mMIMO) systems are essential for 5G/6G networks to meet high throughput and reliability demands, with machine learning (ML)-based techniques, particularly autoencoders (AEs), showing promise for practical deployment. However, standard AEs struggle under noisy channel conditions, limiting their effectiveness. This work introduces a Vector Quantization-based generative AE model (VQ-VAE) for robust mMIMO cross-antenna channel prediction. We compare Generative and Predictive AE-based models, demonstrating that Generative models outperform Predictive ones, especially in noisy environments. The proposed VQ-VAE achieves up to 15 [dB] NMSE gains over standard AEs and about 9 [dB] over VAEs. Additionally, we present a complexity analysis of AE-based models alongside a diffusion model, highlighting the trade-off between accuracy and computational efficiency.

==> acronyms.tex <==
\begin{acronym}
 \acro{AWGN}{additive white Gaussian noise}
 \acro{BER}{bit error rate}
 \acro{BLER}{block error rate}
 \acro{SER}{symbol error rate}
 \acro{DL}{deep learning}
 \acro{GPU}{graphic processing unit}
 \acro{ISI}{inter-symbol interference}
 \acro{LOS}{line-of-sight}
 \acro{MIMO}{multiple-input multiple-output}
 \acro{ML}{machine learning}
 \acro{MLP}{multilayer perceptron}
 \acro{MSE}{mean squared error}
 \acro{NN}{neural network}
 \acro{QAM}{quadrature amplitude modulation}
 \acro{ReLU}{rectified linear unit}
 \acro{SNR}{signal-to-noise ratio}	
 \acro{LLR}{log-likelihood ratio}
 \acro{AE}{autoencoder}
 \acro{ECC}{error correction code}
 \acro{FEC}{forward error correction}
 \acro{LDPC}{low-density parity-check}
 \acro{TX}{transmitter}
 \acro{RX}{receiver}
 \acro{DNN}{deep neural network}
 \acro{CE}{cross entropy}
 \acro{KL}{Kullback-Leibler}
 \acro{wrt}[w.r.t.\@]{with respect to} 
 \acro{i.i.d.}{independent and identically distributed}
 \acro{MMSE}{minimum mean square error}
\end{acronym}

